IoT-LM: Large Multisensory Language Models for the Internet of Things

The Internet of Things (IoT) network integrating billions of smart physical devices embedded with sensors, software, and communication technologies is a critical and rapidly expanding component of our modern world. The IoT ecosystem provides a rich source of real-world modalities such as motion, thermal, geolocation, imaging, depth, sensors, and audio to recognize the states of humans and physical objects. Machine learning presents a rich opportunity to automatically process IoT data at scale, enabling efficient inference for understanding human wellbeing, controlling physical devices, and interconnecting smart cities. To realize this potential, we introduce IoT-LM, an open-source large multisensory language model tailored for the IoT ecosystem. IoT-LM is enabled by two technical contributions: the first is MultiIoT, the most expansive unified IoT dataset to date, encompassing over 1.15 million samples from 12 modalities and 8 tasks prepared for multisensory pre-training and instruction-tuning. The second is a new multisensory multitask adapter layer to condition pre-trained large language models on multisensory IoT data. Not only does IoT-LM yield substantial improvements on 8 supervised IoT classification tasks, but it also demonstrates new interactive question-answering, reasoning, and dialog capabilities conditioned on IoT sensors. We release IoT-LM's data sources and new multisensory language modeling framework.

==> SECTIONS/Experiments/exp_heterogeneity.tex <==
\begin{table}[t]
\centering
\caption{Quantitative results on the heterogeneity in structure and noise.}
 % \vspace{-1.0em}
\label{tab: exp_heterogeneity}
\scalebox{0.75}{
\begin{tabular}{ccccc}
    \toprule
    Noise & Gaze estimation & Depth est. & Touch contact classification & Event detection \\
    \midrule
    IMU & & -- \\
    capacitance & -- & \\
    depth &  \\
    image & \\
    \bottomrule
\end{tabular}}
% \vspace{-1.5em}
\end{table}


==> SECTIONS/Experiments/exp_longrange.tex <==

\begin{wrapfigure}{r}{0.6\textwidth}
\centering
\vspace{-4mm}
% \fbox{\rule{0pt}{2in}
% \rule{0.6\linewidth}{0pt}}
\includegraphics[width=0.92\linewidth]{figs/length_noise_image.png}
\vspace{-0mm}
\caption{Long-range multimodal interactions and heterogeneity between modalities due to noise and imperfections make the \names\ benchmark particularly challenging for ML models.}
\vspace{-0mm}
\label{fig: ablations}
\end{wrapfigure}
